Revisiting Parameter-Efficient Tuning: Are We Really There Yet?

Parameter-Efficient Tuning (PETuning) methods have been deemed by many as the new paradigm for using pretrained language models (PLMs). By tuning just a fraction amount of parameters comparing to full model finetuning, PETuning methods claim to have achieved performance on par with or even better than finetuning. In this work, we take a step back and re-examine these PETuning methods by conducting the first comprehensive investigation into the training and evaluation of them. We found the problematic validation and testing practice in current studies, when accompanied by the instability nature of PETuning methods, has led to unreliable conclusions. When being compared under a truly fair evaluation protocol, PETuning cannot yield consistently competitive performance while finetuning remains to be the best-performing method in medium- and high-resource settings. We delve deeper into the cause of the instability and observed that the number of trainable parameters and training iterations are two main factors: reducing trainable parameters and prolonging training iterations may lead to higher stability in PETuning methods.

==> emnlp2022/author_response.tex <==
\section{Author Response}
We  would like to thank all reviewers for their careful and detailed reading of our paper, as well as their insightful comments. 

% As a summary, our work focuses on the performance and stability of off-the-shelf PETuning methods. We also point out a faulty setting that applying early stopping on the actual test set. 
\subsection{Response to Meta}

\noindent
\textbf{Q1:} \textit{PETuning has its own value considering the current model sizes become extremely huge.}

\noindent
\textbf{A1:} We agree with this perspective that PETuning methods have more parameter efficiency and have mentioned it in Section 3.2. While in this work, we mainly aim to fully compare the performance and stability of PETuning with finetuning, without considering more about the parameter efficiency.


\subsection{Response to Reviewer WbYm}
\noindent
\textbf{Q1:} \textit{Experiments in Section 2 are done with a single model (RoBERTa-base) and a single dataset (RTE dataset that is included in GLUE and SuperGLUE benchmarks).}

\noindent
\textbf{A1:} Intuitively, reusing the test set multiple times during training stage by early stopping has leaked the test information, namely it is a problematic setting. In our experiments, We choose the RTE task as the representative to help to perceive this issue. We would also consider to experiment on more tasks in the revised version.



\subsection{Response to Reviewer DfmS}
\textbf{Q1:} \textit{What results the authors can get by early-stopping \& reporting on the entire test (original dev) set.}

\noindent
\textbf{A1:} We do not report such results in our experiments, but previous work, i.e., P-tuning v2,  has reported the result on RTE task with such settings and has shown that it has many performance "gains" compared with finetuning. To obtain more compelling conclusions, we would redo this experiment for more PETuning methods and report the results in the revised version.

\noindent
\textbf{Q2:} \textit{Some of the works this paper mentions and compares don’t seem to adopt the said problematic evaluation setting, or at least it’s unclear if they do, despite my best attempt to check.}

\noindent
\textbf{A2:} We have cited all PETuning methods that adopt the problematic evaluation setting in Section 2. While the methods we do not specifically mention, like LoRA and BitFit, adopt the regular settings (submitting the test results to GLUE and SuperGLUE benchmarks).

\noindent
\textbf{Q3:} \textit{Perhaps with larger model sizes where FT is even more prone to overfitting, PETuning can do better and achieve their promise of beating FT in even larger data sizes?}

\noindent
\textbf{A3:} This is an intriguing question and it is worth to investigate in future work. While our experiments and conclusions are still helpful for investigating the performance and stability of PETuning methods with different model sizes or types.


\subsection{Response to Reviewer A2W9}
\noindent
\textbf{Q1:} \textit{One could argue there is no novel methodological contribution of this paper. While this might be true, I don’t think papers of this sort should be penalized solely for a lack of methodological novelty.As a practitioner in the NLP field, I find scientific validation and comparison of pre-existing ideas in a rigorous fashion is just as valuable as the presentation of new ideas.}

\noindent
\textbf{A1:} Thanks for the positive review. We also hope that our findings could facilitate more future works about parameter-efficient tuning.


